Master's Thesis: Out-of-distribution Detection with Energy-based Models

Today, deep learning is increasingly applied in security-critical situations such as autonomous driving and medical diagnosis. Despite its success, the behavior and robustness of deep networks are not fully understood yet, posing a significant risk. In particular, researchers recently found that neural networks are overly confident in their predictions, even on data they have never seen before. To tackle this issue, one can differentiate two approaches in the literature. One accounts for uncertainty in the predictions, while the second estimates the underlying density of the training data to decide whether a given input is close to the training data, and thus the network is able to perform as expected.In this thesis, we investigate the capabilities of EBMs at the task of fitting the training data distribution to perform detection of out-of-distribution (OOD) inputs. We find that on most datasets, EBMs do not inherently outperform other density estimators at detecting OOD data despite their flexibility. Thus, we additionally investigate the effects of supervision, dimensionality reduction, and architectural modifications on the performance of EBMs. Further, we propose Energy-Prior Network (EPN) which enables estimation of various uncertainties within an EBM for classification, bridging the gap between two approaches for tackling the OOD detection problem. We identify a connection between the concentration parameters of the Dirichlet distribution and the joint energy in an EBM. Additionally, this allows optimization without a held-out OOD dataset, which might not be available or costly to collect in some applications. Finally, we empirically demonstrate that Energy-Prior Network (EPN) is able to detect OOD inputs, datasets shifts, and adversarial examples. Theoretically, EPN offers favorable properties for the asymptotic case when inputs are far from the training data.

==> chapters/00_backup.tex <==

Use with pdfLaTeX and Biber.

\section{Section}
Citation test (with Biber)~\parencite{latex}.

\subsection{Subsection}

See~\autoref{tab:sample}, \autoref{fig:sample-drawing}, \autoref{fig:sample-plot}, \autoref{fig:sample-listing}, \autoref{fig:tum}, \autoref{fig:tumslide}.

\begin{table}[htpb]
  \caption[Example table]{An example for a simple table.}\label{tab:sample}
  \centering
  \begin{tabular}{l l l l}
    \toprule
      A & B & C & D \\
    \midrule
      1 & 2 & 1 & 2 \\
      2 & 3 & 2 & 3 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}[htpb]
  \centering
  % This should probably go into a file in figures/
  \begin{tikzpicture}[node distance=3cm]
    \node (R0) {$R_1$};
    \node (R1) [right of=R0] {$R_2$};
    \node (R2) [below of=R1] {$R_4$};
    \node (R3) [below of=R0] {$R_3$};
    \node (R4) [right of=R1] {$R_5$};

    \path[every node]
      (R0) edge (R1)
      (R0) edge (R3)
      (R3) edge (R2)
      (R2) edge (R1)
      (R1) edge (R4);
  \end{tikzpicture}
  \caption[Example drawing]{An example for a simple drawing.}\label{fig:sample-drawing}
\end{figure}

\begin{figure}[htpb]
  \centering

  \pgfplotstableset{col sep=&, row sep=\\}
  % This should probably go into a file in data/
  \pgfplotstableread{
    a & b    \\
    1 & 1000 \\
    2 & 1500 \\
    3 & 1600 \\
  }\exampleA
  \pgfplotstableread{
    a & b    \\
    1 & 1200 \\
    2 & 800 \\
    3 & 1400 \\
  }\exampleB
  % This should probably go into a file in figures/
  \begin{tikzpicture}
    \begin{axis}[
        ymin=0,
        legend style={legend pos=south east},
        grid,
        thick,
        ylabel=Y,
        xlabel=X
      ]
      \addplot table[x=a, y=b]{\exampleA};
      \addlegendentry{Example A};
      \addplot table[x=a, y=b]{\exampleB};
      \addlegendentry{Example B};
    \end{axis}
  \end{tikzpicture}
  \caption[Example plot]{An example for a simple plot.}\label{fig:sample-plot}
\end{figure}

\begin{figure}[htpb]
  \centering
  \begin{tabular}{c}
  \begin{lstlisting}[language=SQL]
    SELECT * FROM tbl WHERE tbl.str = "str"
  \end{lstlisting}
  \end{tabular}
  \caption[Example listing]{An example for a source code listing.}\label{fig:sample-listing}
\end{figure}

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{tum}
  \caption[Something else can be written here for listing this, otherwise the caption will be written!]{Includegraphics searches for the filename without extension first in logos, then in figures.} \label{fig:tum}
\end{figure}

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/tum}
  \caption{For pictures with the same name, the direct folder needs to be chosen.} \label{fig:tumslide}
\end{figure}

\begin{figure}[!tbp]
  \centering
  \subfloat[TUM Logo][The logo.]{\includegraphics[height=0.2\textheight]{tum}\label{fig:tum1}}
  \hfill
  \subfloat[TUM Slide][The famous slide.]{\includegraphics[height=0.2\textheight]{figures/tum}\label{fig:tum2}}
  \caption{Two TUM pictures side by side.}
  \label{fig:sidebyside}
\end{figure}

This is how the glossary will be used.

\Glspl{ddye}, \gls{r0}, \gls{R0}, and \gls{kdeac}. Also, the \glspl{tum} has many \glspl{computer}, not only one \Gls{computer}. Subsequent acronym usage will only print the short version of \glspl{tuma} (take care of plural, if needed!), like here with \gls{tuma}, too. It can also be --> \glsdisp{tum}{hidden}\footnote{Example for a hidden TUM glossary entry.} <--.

\todo{Now it is your turn to write your thesis.

This will be a few tough weeks.}

\done{Nevertheless, celebrate it when it is done!}

\begin{table}[]
    \centering
\begin{tabular}{llllll}
\toprule
                & OOD Dataset &       constant & gaussian noise &    segment-ood & uniform noise \\
config.output\_folder & score &                &                &                &               \\
\midrule
\multirow{3}{*}{ce baseline} & differential entropy &  67.94 (16.47) &   53.84 (3.74) &  53.58 (12.53) &  68.74 (4.32) \\
                & max p(y|x) &   41.32 (7.77) &   41.76 (3.01) &   42.35 (8.43) &  36.61 (2.34) \\
                & p(x) &    35.16 (5.3) &   34.47 (0.82) &   37.52 (7.37) &   31.21 (0.2) \\
\cline{1-6}
mcmc & p(x) &   91.45 (3.79) &   86.05 (3.73) &   98.13 (2.24) &  95.83 (2.16) \\
mcmc supervised & p(x) &    98.75 (2.5) &   98.89 (1.25) &  89.18 (18.69) &  99.98 (0.03) \\
vera & p(x) &    100.0 (0.0) &    100.0 (0.0) &  87.34 (17.69) &   100.0 (0.0) \\
vera supervised & p(x) &   99.97 (0.05) &   99.99 (0.02) &  84.56 (16.46) &   100.0 (0.0) \\
\bottomrule
\end{tabular}

    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> pages/acknowledgements.tex <==
\makeatletter
\ifthenelse{\pdf@strcmp{\languagename}{english}=0}
{\addcontentsline{toc}{chapter}{Acknowledgments}}
{\addcontentsline{toc}{chapter}{Danksagungen}}
\makeatother
\thispagestyle{empty}

\vspace*{20mm}

\begin{center}
\makeatletter
\ifthenelse{\pdf@strcmp{\languagename}{english}=0}
{\usekomafont{section} Acknowledgments}
{\usekomafont{section} Danksagungen}
\makeatother
\end{center}

\vspace{10mm}

%TODO: Acknowledgments

\cleardoublepage{}

